Axiomatizing Origami planes

We provide a variant of an axiomatization of elementary geometry based on logical axioms in the spirit of Huzita--Justin axioms for the Origami constructions. We isolate the fragments corresponding to natural classes of Origami constructions such as Pythagorean, Euclidean, and full Origami constructions. The sets of Origami constructible points for each of the classes of constructions provides the minimal model of the corresponding set of logical axioms. Our axiomatizations are based on Wu's axioms for orthogonal geometry and some modifications of Huzita--Justin axioms. We work out bi-interpretations between these logical theories and theories of fields as described in J.A. Makowsky (2018). Using a theorem of M. Ziegler (1982) which implies that the first order theory of Vieta fields is undecidable, we conclude that the first order theory of our axiomatization of Origami is also undecidable.

==> background-rev.tex <==
\section{Background on geometry}
\label{se:background}
Our axiomatization uses
%is based on the standard  approach with
two basic sorts of variables, denoting lines and points, respectively.
We use $P, P_1, \ldots, P_i$, and more liberally, upper case letters, to denote points and
$\ell, \ell_1, \ldots, \ell_i$, and more liberally, lower case letters, to denote lines.

In our axiomatization we use the following basic relations:
\begin{enumerate}[(i)]
\item
the \emph{incidence} relation
$ P \in \ell$ between points and lines,
\item
the \emph{orthogonality} relation $\ell_1 \perp \ell_2$ between two lines,
%\item the equidistance relation between two pairs of points $P_1, P_2$ and $Q_1, Q_2$ denoted by $P_1P_2 \cong q_1q_2$.
\item
and the \emph{betweenness} (or \emph{order}) relation between three points $P_1, P_2, P_3$ denoted by
$Be(P_1, P_2, P_3)$.
\end{enumerate}

The sorts are, however, definable using the incidence relation:
$\ell$ is a line iff $\exists P (P \in \ell)$,
and
$P$ is a point iff $\exists \ell (P \in \ell)$. We also note that the equidistance relation $PQ\cong RS$ between points $P,Q$
and $R,S$ is definable from incidence and orthogonality~\cite[page 25]{bk:Wu1994}.

%Our approach is inspired by
We start with
Wu's axiomatization of orthogonal geometry, cf.~\cite{bk:Wu1994},
augmented by the axioms for betweenness, and
%Most of our basic axioms come from Wu's axiomatization of orthogonal geometry,
%to which we add
appropriate versions of Huzita--Justin axioms.
We denote
by $\tau_{wu}$ the vocabulary corresponding to (i)-(ii)
and
by $\tau_{o-wu}$ the vocabulary corresponding to (i)-(iii). By
$\FOL(\tau_{wu})$
and
$\FOL(\tau_{o-wu})$ we denote
the corresponding sets of first order formulas.

The Huzita -- Justin axioms (H-1), (H-2), (H-4)  can be used as they are.
However, we modify axioms (H-3), (H-5), (H-6) to (H*3), (H*5), (H*6) in a way to assure that they are always applicable.
The axioms (H-1), (H-2), (H*3), (H-4), (H*6)  can be formulated in $\FOL(\tau_{wu})$.
In order to formulate (H*5) we use the betweenness relation.

As the most general class of structures for our study we consider \emph{metric Wu planes} (see \cite{makowsky2019can}).
Metric Wu planes already satisfy Huzita -- Justin axioms (H-1), (H-2), (H*3), (H-4),
where axiom (H-3) is modified so that it holds more generally in arbitrary metric Wu planes rather than just in the ordered ones.
Then we add to the axioms of metric Wu planes the axioms of betweenness and further origami axioms (H*5),
(H*6) and obtain the corresponding classes of structures. See Section \ref{wuplanes}
for the list of axioms used in the definitions below.

\begin{definition} \mbox{}
\begin{enumerate}[(i)]
\item
A $\tau_{wu}$-structure $\Pi$ is a {\em metric Wu plane}
if it satisfies (I-1), (I-2), (I-3), (O-1), $\ldots$,  (O-5),
the axiom of infinity (InfLines), (ParAx), the two axioms of Desargues (De-1) and (De-2) and (AxSymAx).
\item
An {\em ordered metric Wu plane} is a metric Wu plane satisfying axioms of order (B-1), $\ldots$, (B-4).
\item
A {\em Euclidean ordered metric Wu plane} is an ordered metric Wu plane satisfying (H*5).
\item
An {\em ordered origami plane} is an ordered metric Wu plane satisfying (H*5) and (H*6).
\end{enumerate}
\end{definition}

Only items (iii) and (iv) involve origami or modified origami axioms in their definitions.

The following theorems are from J.A. Makowsky \cite{makowsky2019can}.
They can be seen as a logical formalization of the classical results on coordinatization
(see \cite{hall1943projective,bk:Wu1994}).
\begin{theorem}
\label{prop:JAM}
\begin{enumerate}[(i)]
\item
The theory of  metric Wu planes is bi-interpretable with the theory of Pythagorean fields of characteristic $0$.
\item
The theory of ordered  metric Wu planes is bi-interpretable with the theory of ordered Pythagorean fields.
\end{enumerate}
\end{theorem}

Ziegler \cite{ar:ziegler} showed that any finitely axiomatized subtheory of the first order theory of real closed fields is undecidable.
One of the main ideas of \cite{makowsky2019can} was the use of this result (via bi-interpretability) to show that certain elementary theories of geometries are undecidable. For example,
as a corollary of Ziegler's theorem one can conclude from Theorem \ref{prop:JAM} that the elementary theories of the classes of metric Wu planes and of ordered metric Wu planes are undecidable.


The main contributions of this paper are as follows.
\begin{theorem}
\label{th:main-1}
\begin{enumerate}[(i)]
\item The theory of Euclidean ordered metric Wu planes is bi-interpretable with the theory of Euclidean fields;
\item The theory of ordered origami planes is bi-interpretable with the theory of Vieta fields.
\end{enumerate}
\end{theorem}

Again, via bi-interpretability, Ziegler's theorem is applicable to both theories, hence both are undecidable.


